Me, Myself and My Killfie: Characterizing and Preventing Selfie Deaths

Over the past couple of years, clicking and posting selfies has become a popular trend. However, since March 2014, 127 people have died and many have been injured while trying to click a selfie. Researchers have studied selfies for understanding the psychology of the authors, and understanding its effect on social media platforms. In this work, we perform a comprehensive analysis of the selfie-related casualties and infer various reasons behind these deaths. We use inferences from incidents and from our understanding of the features, we create a system to make people more aware of the dangerous situations in which these selfies are taken. We use a combination of text-based, image-based and location-based features to classify a particular selfie as dangerous or not. Our method ran on 3,155 annotated selfies collected on Twitter gave 73% accuracy. Individually the image-based features were the most informative for the prediction task. The combination of image-based and location-based features resulted in the best accuracy. We have made our code and dataset available at http://labs.precog.iiitd.edu.in/killfie.

==> dfn.tex <==
\newtheorem{observation}{Observation}
\newtheorem{conjecture}{Conjecture}
\newtheorem{problem}{Problem}
\newtheorem{algo}{Algorithm}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{theorem}{Theorem}
\newtheorem{question}{Question}
\newtheorem{example}{Example}
\newtheorem{answer}{Answer}
\newtheorem{proof}{Proof}

\newcommand{\hide}[1]{}
\newcommand{\notice}[1]{{\textsf{\textcolor{green}{{\em [#1]}}}}}
\newcommand{\reminder}[1]{{\textsf{\textcolor{red}{[#1]}}}}
\newcommand{\vectornorm}[1]{\left|\left|#1\right|\right|}

\newcommand{\mkclean}{
    \renewcommand{\reminder}{\hide}
}

% from cf: shorthands - also they make tighter lists
% \newcommand{\bit}{\begin{itemize*}}
% \newcommand{\eit}{\end{itemize*}}
% \newcommand{\ben}{\begin{enumerate*}}
% \newcommand{\een}{\end{enumerate*}}
\newcommand{\bit}{\begin{compactitem}}
\newcommand{\eit}{\end{compactitem}}
\newcommand{\ben}{\begin{compactenum}}
\newcommand{\een}{\end{compactenum}}

\newcommand{\QED}{ \hfill {\bf QED}}
\newcommand{\method}{\textsc{DetFi}\xspace}

\newcommand{\douli}{\textsc{Douli}}
\newcommand{\mapreduce}{\textsc{MapReduce}\xspace}
\newcommand{\hadoop}{\textsc{Hadoop}\xspace}
\newcommand{\nodeiterator}{\textsc{NodeIterator}\xspace}
\newcommand{\edgeiterator}{\textsc{EdgeIterator}\xspace}
\newcommand{\doulinodeiterator}{\textsc{DouliNodeIterator}\xspace}
\newcommand{\eigen}{\textsc{EigenTriangle}\xspace}

